ScreenLLM: Stateful Screen Schema for Efficient Action Understanding and Prediction

Graphical User Interface (GUI) agents are autonomous systems that interpret and generate actions, enabling intelligent user assistance and automation. Effective training of these agent presents unique challenges, such as sparsity in supervision signals, scalability for large datasets, and the need for nuanced user understanding. We propose stateful screen schema, an efficient representation of GUI interactions that captures key user actions and intentions over time. Building on this foundation, we introduce ScreenLLM, a set of multimodal large language models (MLLMs) tailored for advanced UI understanding and action prediction. Extensive experiments on both open-source and proprietary models show that ScreenLLM accurately models user behavior and predicts actions. Our work lays the foundation for scalable, robust, and intelligent GUI agents that enhance user interaction in diverse software environments.

==> src/backup_method.tex <==
\paragraph{Long-term Memory} 
Inferring user intentions usually require inputs from all previous actions. We equip models with long-term video modeling capability using a memory module based on an LSTM network.
\begin{align}
    \mathbf{h}_t, \mathbf{c}_t &= \mathrm{LSTM}(x_{t}, \mathbf{h}_{t-1}, \mathbf{c}_{t-1}), \\
    \mathbf{h}_0 &= \mathbf{c}_t = \mathbf{0}.
\end{align}
where $\mathbf{h}_t$ is the hidden state at the current time step $t$ that encapsulates the long-term memory from all previous clips in the same video. $\mathbf{c}_t$ is the cell vector.

We use attention to query useful information from the hidden states of the LSTM: 
\begin{eqnarray}
\label{eq:kernel_match_1}
\mathbf{Q}_t=\mathbf{z} \mathbf{W}_Q, \mathbf{K}_t=\textbf{h}_t \mathbf{W}_K, \mathbf{V}_t=\textbf{h}_t \mathbf{W}_V,
\end{eqnarray}
where $\textbf{z}$ is a trainable parameter that is used to query useful information from all previous clips in the video. $\mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V$ are the weights of the attention module. 

Then we apply the cross-attention operation as:

\begin{align}
\textbf{O}_t &=\mathrm{Attn}(\textbf{Q}_t, \textbf{K}_t, \textbf{V}_t)   \\
&=\mathrm{Softmax}\left(\frac{\textbf{Q}_t \textbf{K}_t^T}{\sqrt{D}}\right) \textbf{V}_t.
\end{align}


The original token representations LLM uses to generate the outputs is 
\begin{equation}
    \textbf{E}_t = \mathrm{Embed}(\{\textbf{f}_{t-1}^i\}, p_t)
\end{equation}
where $p_t$ is the textual prompt at time $t$.

($p$ does not need to change w.r.t timestamp, but tasks)

Finally, we interpolate $\textbf{O}_t$ and the hidden states. 
\begin{align}
\textbf{E}_t' &= \alpha \textbf{E}_t + (1 - \alpha) \textbf{O}_t \quad & \text{if} \, &t \ge 1, \\
\textbf{E}_t^{\prime} & = \textbf{E}_t \quad & \text{if} \, t = 0.
\end{align}
where $\alpha \in [0, 1]$ is a hyperparameter. The interpolated embeddings $\textbf{E}_t'$ is then used as inputs to the LLM.

\paragraph{LLM Generation}
During generation, we feed the inputs, including textual prompt $p_t$, aligned representations of the visual inputs $\mathbf{f}_t^i$, and screen schema.  to our multimodal LLM (MLLM)~\cite{liu2023improved,liu2023visual} to derive both the answer $a$ and the hidden states of the LLM $\textbf{E}_t$:
\begin{align} 
    a_t, \textbf{E}_t & = \mathrm{LLM}(\textbf{E}_{t-1}', s_{t-1})
\end{align}

\yq{Note the terminologies here. e.g. LLM vs. MLLM, token representations}

where $s_t$ is the screen schema. $\mathbf{E}_t \in \mathbb{R}^{Q \times D}$ is the hidden states of the LSTM, and $D$ is the dimension of the embedding.

% First, we use the LLM backbone to generate the answers based on the textual prompt, aligned representations of the visual inputs, and screen schema. 

\clearpage
\begin{verbatim}
for (timestamp t, clip c_t) in long_video:

    [f_t^0, ..., f_t^9] = FrameSampler(v_t)

    # For each frame, generate a screen schema
    for i in range(10):
        s_t^i = SchemaGenerator(f_t^i)
    endfor

    
    # B: Batch size
    # Q: Number of queries
    # D: Hidden dimension

    # Initialize the hidden and cell states at the first timestamp
    if t == 0:
        h_t = zeros(B, Q * D)  # Initialize the hidden state
        c_t = zeros(B, Q * D)  # Initialize the cell state
        E_t' = Embed({f_t^i}, p_t)

    else:
        O_t = Attention(z.dot(W_Q), h_t.dot(W_K), h_t.dot(W_V))
        E_t' = alpha * E_t + (1 - alpha) * O_t
    endif

    # Get the multimodal LLM's answer a_t and hidden states E_t
    a_t, E_t = MLLM(, screen_schema {s_t^i}, )
    
    # Update LSTM parameters using the current output and previous states
    
    h_{t+1}, c_{t+1} = LSTMCell(Project(E_t), h_t, c_t)

endfor

    
\end{verbatim}
